A Parallel Low-Rank Solver for the Six-Dimensional Vlasov-Maxwell Equations

Continuum Vlasov simulations can be utilized for highly accurate modelling of fully kinetic plasmas. Great progress has been made recently regarding the applicability of the method in realistic plasma configurations. However, a reduction of the high computational cost that is inherent to fully kinetic simulations would be desirable, especially at high velocity space resolutions. For this purpose, low-rank approximations can be employed. The so far available low-rank solvers are restricted to either electrostatic systems or low dimensionality and can therefore not be applied to most space, astrophysical and fusion plasmas. In this paper we present a new parallel low-rank solver for the full six-dimensional electromagnetic Vlasov-Maxwell equations with a compression of the particle distribution function in velocity space. Special attention is paid to mass conservation and Gauss's law. The low-rank Vlasov solver is applied to standard benchmark problems of plasma turbulence and magnetic reconnection and compared to the full grid method. It yields accurate results at significantly reduced computational cost.

==> moment_fitting.tex <==

Every truncation of the distribution function is accompanied by a
small error which breaks the conservation properties that a Vlasov
scheme can have without low-rank approximation. In particular,
the low-rank version of the PFC scheme does no longer conserve
mass. This is of course problematic for the physical reliability
of the simulation, but also for the interplay of the Vlasov solver and the Maxwell
solver. The FDTD Maxwell solver is designed to fulfill Gauss's law
$\nabla \cdot \mathbf{E} = \rho / \epsilon_0$ at any time, if it
is fulfilled initially. However, this is not anymore possible when
the charge density $\rho$ is not conserved. A simple rescaling of $f$ before the
Maxwell step in order to conserve total charge density does improve the
situation but is no sufficient solution -- there are still
local errors in $\rho$.

To conserve mass in the low-rank Vlasov solver, it is combined with
a partial differential equation (PDE) fluid solver using moment fitting
\citep{rieke-trost-grauer:2015,trost-lautenbach-grauer:2017,allmann-rahn-lautenbach-grauer:2021};
a simpler version of the dual Vlasov solver that was introduced in this thesis.
The dual Vlasov solver in Sec.~\ref{sec:dual_vlasov_solver} is based
on an exchange of the ten moment Maxwellian part of the distribution
function with the ten moment Maxwellian obtained from the fluid solver.
In low-rank format this is not possible at good performance because
the ten moment Maxwellian mixes two velocity space directions
and therefore does not separate. It cannot be constructed directly
in low-rank format and a truncation starting from the full tensor
in each time step is much too costly. Thus, an alternative approach
will be employed here where only density and mean velocity are
corrected by the fluid solver. A time step of the dual low-rank
Vlasov solver, as implemented, is described in Algorithm~\ref{alg:timestep_dual_lrv}.

\begin{algorithm}
\SetAlgoLined
 \Timestep{}{
  Half step of Maxwell solver\\
  Calculate second moment $\mathcal{P}^{t}$ from $f^t$\\
  Full Vlasov Leapfrog Step to advance to $f^{t+1}$\\
  Calculate $\mathcal{P}^{t+1}$ from $f^{t+1}$\\
  Interpolate to get $\mathcal{P}^{t+1/2}$\\
  Full Runge-Kutta Fluid Step (input $\mathcal{P}$ at appropriate times)\\
  \Momentfitting{}{
    Calculate mean velocity $\mathbf{u}_{\text{V}}$ from $f$\\
    Artificial advection step with advection velocity $\mathbf{u}_{\text{V}}-\mathbf{u}_{\text{F}}$
    to enforce $\mathbf{u}_{\text{V}}=\mathbf{u}_{\text{F}}$\\
    Calculate density $n_{\text{V}}$ from $f$\\
    Rescale $f$ by $n_{\text{F}}/n_{\text{V}}$ to conserve mass\\
  }
  Second half step of Maxwell solver\\
 }
 \caption{Time stepping of the low-rank Vlasov-Maxwell solver with moment fitting}
 \label{alg:timestep_dual_lrv}
\end{algorithm}

In this version of the moment fitting a four moment fluid solver is used
where the hierarchy of fluid equations is closed at the
momentum equation \eqref{eq:tenmoment_movement} using the second moment
tensor $\mathcal{P}$ obtained from the distribution function. Then the fluid solver
yields solutions for $n$ and $\mathbf{u}$, but not for the energy, and only
these moments can be used to correct the distribution function. In contrast to
the full grid dual solver, now the density of the Vlasov solver is not conserved
and is therefore corrected by the solution from the PDE solver. The correction
of the mean velocity does not happen via an exchange of Maxwellians, but through
an artificial advection step which moves the Vlasov solution towards the
solution from the PDE solver. This method was first used in \citep{rieke-trost-grauer:2015}
for spatial coupling of Vlasov and fluid models. For a non-positive scheme
like the low-rank scheme here, the advection method has the advantage that
it does not introduce additional negativity caused by the exchange of Maxwellians.
Since the four moment fluid solver does not yield a solution for the energy
tensor, energy is not included in moment fitting and total energy is not
conserved in the resulting low-rank dual Vlasov solver. However, the low-rank
method allows much higher velocity space resolutions than the full grid solver
and therefore also has less issues with numerical heating.

In the future one way to apply energy conserving moment fitting to the
low-rank solver could be to compute the standard Maxwellian \eqref{eq:maxwell_distribution}
from both $f$ and the ten moment solution and exchange these standard
Maxwellians. This is easily possible in low-rank format. After this
correction, however, the second moment solution $\mathcal{P}_\text{F}$
from the fluid solver must be replaced with the solution $\mathcal{P}_\text{V}$ obtained
from the distribution function in order to have consistent solutions. This method
is rather keen and it must be checked whether it causes small artificial temperature anisotropies.
Furthermore, the moment fitting based on the exchange of Maxwellians can become unstable
at large positivity violations, so the primary challenge is to avoid or reduce
non-positivity of the low-rank solver.



==> stepx.tex <==
For the numerical solution of the Vlasov equation we employ a semi-Lagrangian
method. In order to simplify the characteristic equation, we apply an operator splitting
and solve the $\mathbf{x}$ and $\mathbf{v}$ steps separately.
In the second-order time splitting that we use, a half velocity space
step (using $\Delta t / 2$ for the update) is followed by a full step
in position space and a second half step in velocity space. This is
also known as the leapfrog method.

First, we discuss the $\mathbf{x}$ advection, i.e. we solve the equation
\begin{equation}
\partial_t f + \mathbf{v} \cdot \nabla_{\mathbf{x}} f = 0. 
\end{equation}
Denoting the value of $f$ at time $t^n$ by $f^n$ and the new
value at time $t^{n+1} = t^n + \Delta t$ by $f^{n+1}$ it is
\begin{equation}
f^{n+1}(\mathbf{x},\mathbf{v}) =
f^{n}\left(\mathbf{x} - \mathbf{v} \Delta t, \mathbf{v} \right).
\label{eq:semi_lagrange_update}\end{equation}

In general $f^{n}\left(\mathbf{x} - \mathbf{v} \Delta t, \mathbf{v}\right)$ is
not available as a grid point and must instead be interpolated.
Many of the available semi-Lagrangian interpolation methods (e.g.~spline
interpolation) can be utilized by a low-rank Vlasov solver as long
as no positivity preserving limiters are involved.
The $x$, $y$ and $z$ directions are independent
for the step in position space so that the update in each direction can simply
be carried out one after the other and a one-dimensional
scheme can be used.
We choose the positive and flux-conservative (PFC) Vlasov scheme
in \cite{filbet-sonnendruecker-bertrand:2001} without limiters since this method
leads to relatively few numerical oscillations. There, the grid points are
not associated with the value of $f$ at that certain point but with the average of $f$ in
the respective cell (or the cell integral). Then the semi-Lagrangian method can be formulated
in terms of fluxes in and out of the cell.
Thus, $f_i$ is now the average value of $f$ within cell $i$ which
is given by
\begin{equation}
f_i^n = \frac{1}{\Delta x} \int^{x_{i+1/2}}_{x_{i-1/2}} f(t^{n},x)\,\D x.
\end{equation}
The solution of the Vlasov equation can be split into one-dimensional
advection steps, so let for now the coordinates besides $x$ be fixed
such that $f^n = f(x,t^n)$. The semi-Lagrangian update of the cell
integral is
\begin{equation}
\int^{x_{i+1/2}}_{x_{i-1/2}} f(t^{n+1},x)\,\D x =
\int^{X(x_{i+1/2})}_{X(x_{i-1/2})} f(t^{n},x)\,\D x
\end{equation}
where $X$ is the origin of the particle trajectory and
$x_{i-1/2} = x_{\text{begin}} + (i-1)\,\Delta x$ is the left border
of the $i$th cell with $x_{\text{begin}}$ the lower limit of position
space in $x$-direction. For example, in the case of an $x$-step it
is $X(x_{i-1/2}) = x_{i-1/2} - v_x \Delta t$. The flux out of
the cell is defined as
\begin{equation}
\Phi_{i+1/2}(t^n) = \int^{x_{i+1/2}}_{X(x_{i-1/2})} f(t^{n},x)\,\D x
\end{equation}
so that the semi-Lagrangian update can be written as
\begin{equation}
\int^{x_{i+1/2}}_{x_{i-1/2}} f(t^{n+1},x)\,\D x =
\Phi_{i-1/2}(t^n) + \int^{x_{i+1/2}}_{x_{i-1/2}} f(t^{n},x)\,\D x - \Phi_{i+1/2}(t^n).
\end{equation}

In the PFC scheme \cite{filbet-sonnendruecker-bertrand:2001} 
the fluxes are obtained from a sum of weighted neighbouring cells. In the low-rank
case these fluxes are calculated with the following implementation.
Let $a = -v_j \Delta t / \Delta x_j$ be the normalized advection velocity
and $\alpha_i = x_{j+1/2} - X(x_{i+1/2})$ where $j$ is the index of the cell in which $X(x_{i+1/2})$ is located.
Then it is $\alpha(v_j) = |a - \integer(a)|$. For $a < 0$ the weights are
\begin{align}
W_1(v_j) &= -\alpha\,(1-\alpha)\,(1+\alpha)\,/6 \nonumber\\
W_2(v_j) &=  \alpha\,\big(1 - (1-\alpha)\,(2-\alpha)\,/6 + (1-\alpha)\,(1+\alpha)\,/6 \big) \nonumber\\
W_3(v_j) &=  \alpha\,(1-\alpha)\,(2-\alpha)\,/6 \nonumber\\
W_4(v_j) &=  0
\end{align}
and for $a > 0$ it is
\begin{align}
W_1(v_j) &=  0 \nonumber\\
W_2(v_j) &= -\alpha\,(1-\alpha)\,(2-\alpha)\,/6 \nonumber\\
W_3(v_j) &= -\alpha\,\big(1 - (1-\alpha)\,(2-\alpha)\,/6 + (1-\alpha)\,(1+\alpha)\,/6 \big) \nonumber\\
W_4(v_j) &=  \alpha\,(1-\alpha)\,(1+\alpha)\,/6.
\end{align}
In the computation of $\alpha$ the $\integer$ function was used which truncates
its argument to a whole number, for example $\integer(1.6) = 1$ and $\integer(-1.6) = -1$.
The flux is given by
\begin{equation}
\Phi_{i-1/2} = f_{i-2}^n W_1 + f_{i-1}^n W_2 + f_{i}^n W_3 + f_{i+1}^n W_4
\label{eq:pfc_weighted_sum}\end{equation}

For the design of the algorithm, the exact form of the weights is irrelevant,
it is only important to note that they depend on the
velocity $v_j$ for an update in direction $x_j,\ j\in \{1,2,3\}$.
The low-rank distribution function $f(\mathbf{x}) \in \mathbb{H}$ is a field of hierarchical Tucker tensors with
explicitly available cells in position space and a compressed velocity space. The interpolation
\eqref{eq:pfc_weighted_sum} can be performed with a compressed $f$. There is no
problem with selecting the cells left and right
to cell $i$ as they can be addressed explicitly in position space.
The sum is carried out for all cells in velocity space so
\eqref{eq:pfc_weighted_sum} can be considered to be a sum of four
third-order velocity space tensors. The only question that remains is how
the weights are applied when the velocity space cells cannot be directly
accessed due to the low-rank decomposition. Fortunately, the factor matrices $\mathrm{U}$ of the hierarchical Tucker
tensors each represent one velocity space direction and the numbers of
rows of the factor matrices corresponds to the chosen velocity space
resolution. The rows are ordered such that the first row is associated
with the lower limit of velocity space, the last row with the upper limit
and steps of $\Delta v$ in between. The weights depend on the discretized
velocity space and can be interpreted as a vector $\mathbf{W} \in \mathbb{R}^{N_j}$,
where $N_j$ is the resolution of velocity space in direction $v_j$.
Then, the multiplication of the distribution function $f$ with a weight $W$
is the element-wise product of the row vectors $\mathbf{U}_{j,k}$ of $f$'s factor
matrix $\mathrm{U}_j$ with the weight vector:
\begin{equation}
\mathbf{U}_{j,k} \star \mathbf{W}, \quad \forall \, k \in \{1,\dots,r_j\}.
\label{eq:U_star_W}\end{equation}
The element-wise product is defined (for tensors of order $d$) as
\begin{equation}
\mathrm{Z}_{i_1 i_2 ... i_d} = (\mathrm{X} \star \mathrm{Y})_{i_1 i_2 ... i_d} =
(\mathrm{X}_{i_1 i_2 ... i_d} \mathrm{Y}_{i_1 i_2 ... i_d})_{i_1 i_2 ... i_d}.
\label{eq:hadamard}\end{equation}
The in this case four weights can be computed once initially for all velocity space
cells, as they do not change with time. Then in every spatial step
in direction $x_j$ the neighbouring weighted hierarchical Tucker tensors
$f_{i-2} W_1 \dots f_{i+1} W_4$ are added up with a truncation in between each
addition to compute the fluxes. Afterwards the new value of $f$ can be obtained as
\begin{equation}
f^{n+1}_i = \Phi_{i-1/2} + f^n - \Phi_{i+1/2}
\end{equation}
which again is a sum of HT tensors with a truncation after each
addition.

The weights have been simplified from the original PFC scheme in order to be
applicable in the low-rank solver. It is not yet clear how the slope
limiters for preserving the positivity of the distribution function
are efficiently applied when $f$ is in
a low-rank format because the cells that are arguments of the minimum function
in the limiter are not explicitly available. Therefore, the limiters are for now turned
off ($\epsilon^+ = \epsilon^- = 1$). This issue persists for all typical slope
limiters, and it is clear that it is non-trivial to prevent negative values
of the distribution function when it is not known which cells
actually violate the positivity. A second simplification made is that 
a CFL number smaller than one is enforced, i.e.\ $a \in (-1,1)$.
For larger CFL numbers additional weights must be introduced. Since the
time step restrictions are more severe for the step in velocity space
in typical  applications of the low-rank Vlasov solver, it is most efficient to
enforce a CFL below one in the step in position space and allow a
CFL below two in the velocity space step.


